Simulating Quantum Materials with Digital Quantum Computers

Quantum materials exhibit a wide array of exotic phenomena and practically useful properties. A better understanding of these materials can provide deeper insights into fundamental physics in the quantum realm as well as advance technology for entertainment, healthcare, and sustainability. The emergence of digital quantum computers (DQCs), which can efficiently perform quantum simulations that are otherwise intractable on classical computers, provides a promising path forward for testing and analyzing the remarkable, and often counter-intuitive, behavior of quantum materials. Equipped with these new tools, scientists from diverse domains are racing towards achieving physical quantum advantage (i.e., using a quantum computer to learn new physics with a computation that cannot feasibly be run on any classical computer). The aim of this review, therefore, is to provide a summary of progress made towards this goal that is accessible to scientists across the physical sciences. We will first review the available technology and algorithms, and detail the myriad ways to represent materials on quantum computers. Next, we will showcase the simulations that have been successfully performed on currently available DQCs, emphasizing the variety of properties, both static and dynamic, that can be studied with this nascent technology. Finally, we work through two examples of how to map a materials problem onto a DQC, with full code included in the Supplementary Material. It is our hope that this review can serve as an organized overview of progress in the field for domain experts and an accessible introduction to scientists in related fields interested in beginning to perform their own simulations of quantum materials on DQCs.

==> notes.tex <==
Bauer Review:

* Focus on digital quanutm computation, as opposed to analog or adiabatic: A more general approach, which is the focus of this review, is digital quan- tum computation. Here, very much in analogy to the classical computers we are used to, one considers a system of quantum registers – qubits – that are controlled through some set of in- structions - the quantum gate operations. One can show that with a finite (and indeed relatively small) set of such gate op- erations, one can in principle generate arbitrary quantum evo- lution to arbitrary precision!

* Use of quantum chemistry: Determining the main features of the resulting potential energy surface, i.e. the electronic energy as a function of nuclear po- sitions, its minima and saddle points, is key to understanding chemical reactivity, product distributions, and reaction rates.

* single-reference vs. multi-reference states. most methods in quantum chem- istry are most accurate for problems where there is a domi- nant electronic configuration. Single- reference quantum chemistry is found in the ground-states of many simple molecules. in many molecular excited states, at stretched bond geometries, and in transition metal chemistry, multiple electronic configurations can come into play. examples of multi-reference quantum chemical problems: The chemistry of enzyme active sites, Transition metal nanocatalysts and surface catalysts, Light harvesting and the vision process. 

* Quantum molecular dy- namics is primarily concerned with the nuclear motion and describes the rates of chemical processes as well as the dy- namical interaction of molecules with light, as involved in spectroscopy and quantum control. sections) and are thus central in describing energy transfer. The faithful de- scription of non-adiabatic quantum effects requires the simul- taneous treatment of quantum electrons and quantum nuclei.

*For these reasons, it remains to be understood whether the quantum algorithms of relevance to quantum chemistry are those of relevance to ma- terials electronic structure. This review will cover quantum computation methods for quantum chemistry since they may be relevant to materials simulations.  These methods currently apply to small molecules, and materials, afterall are comprised of small molecules. Thus in a brute force manner, quantum chemistry methods can be extended to materials simulations.  reasons materials simulations can be simpler include the fact that often very simple Hamiltonians describe the main physics, as well as the potential presence of translational invariance




notes to mention:

*importance of planewave-based methods for materials simulations

Materials design has emerged as one of the great challenges of the twenty-first century.  Given the huge demand for smaller, faster, and lower-power devices with potential for favorable capabilities such as flexibility and transparency, the need to find new materials for such improvements is paramount.  Integrating a new material into electronic devices, however, requires a detailed understanding of how it behaves at the molecular level, within the realm of quantum mechanics. 

\begin{table}
\caption{\label{HardwareTable}Table of advanced quantum hardware technologies and their ranges for benchmark attributes. \cite{xiang2013hybrid, Wendin:2017, YenHsiang:2018}}.
\footnotesize
\rowcolors{2}{gray!25}{white}
\begin{tabular}{ | m{7em} | m{7em}| m{9em} | m{7em} | m{9em} |}
\br
\rowcolor{gray!50}
\textbf{Technology}&\textbf{Qubit Count}&\textbf{Coherence Time [s]}&\textbf{Gate Speed [s]}&\textbf{Gate Fidelity [\%]}\\
Superconducting qubits & 20-70 & $10^{-6}$--$10^{-5}$ &
$10^{-8}$--$10^{-7}$ & 96.5-99.4 \\
Trapped-ion qubits & 32 & $10^{-1}$ & $10^{-7}$--$10^{-4}$ & 97-99.9999\%  \\
\br
\end{tabular}\\
\end{table}
\normalsize

They can be categorized into families based on the underlying operation that can be performed more efficiently on quantum computers than on classical computers. The family based on quantum Fourier transform includes Shor's algorithm for factoring integers in polynomial time~\cite{Shor:1997}. The family based on the amplitude amplification algorithm includes Grover's database search algorithm~\cite{Grover:1997}. Algorithms in this family offer quadratic speedup over classical algorithms. Hybrid algorithms that combine both quantum and classical processing represent yet another family. An example is the quantum approximate optimization algorithm for solving combinatorial problems~\cite{Farhi:2014}.




The limiting factors of current quantum technologies are environment noise and qubit connectivity. Environment noise decreases coherence times and reduces gate fidelities. It can be mitigated by engineering improvements, by error mitigation algorithms, and also by designing algorithms with lower gate depth. 
The quantum speedup is closely related to the number of the so-called $T$ gates in a quantum circuit. However, $T$ gates are also the most difficult gates to implement within error-correcting codes. Methods that limit their total number are being actively developed~\cite{Babbush:2018b}.

Limited qubit connectivity restricts qubit operations only to qubits that are directly connected in the hardware. Usually, each qubit is coupled only to a few of its neighboring qubits. It is then important to analyze if the proposed algorithms are scalable in architectures with limited connectivity. Recent work has shown that the Suzuki--Trotter factorization is efficient even in linearly connected architectures~\cite{Kivlichan:2018}. 
\\
\textbf{This section below seems to better fit in 4.1 or thereabouts}
Another related problem are many-orbital interactions in interesting Hamiltonians. Quantum computers typically support only two-qubit gates. However, it is possible to approximately map any many-body interaction Hamiltonian to two-body Hamiltonian using the concept of perturbative gadgets~\cite{Kempe:2006, Jordan:2008, Bravyi:2008, Babbush:2014}.


% \subsection{Algorithmic improvements}

% The limiting factors of current quantum technologies are environment noise and qubit connectivity. Environment noise decreases coherence times and reduces gate fidelities. It can be mitigated by engineering improvements, by error mitigation algorithms, and also by designing algorithms with lower gate depth. It is possible to decrease the number of terms in the Hamiltonian from $\mathcal{O}(N^4)$ to $\mathcal{O}(N^2)$, where $N$ is the number of spin-orbitals, by using alternative basis sets instead of ordinary Gaussian basis sets~\cite{Babbush:2018a}. The circuit depth of a Trotter--Suzuki step then scales linearly with $N$~\cite{Kivlichan:2018}. The quantum speedup is closely related to the number of the so-called $T$ gates in a quantum circuit. However, $T$ gates are also the most difficult gates to implement within error-correcting codes. Methods that limit their total number are being actively developed~\cite{Babbush:2018b}.

% Limited qubit connectivity restricts qubit operations only to qubits that are directly connected in the hardware. Usually, each qubit is coupled only to a few of its neighboring qubits. It is then important to analyze if the proposed algorithms are scalable in architectures with limited connectivity. Recent work has shown that the Suzuki--Trotter factorization is efficient even in linearly connected architectures~\cite{Kivlichan:2018}. Another related problem are many-orbital interactions in interesting Hamiltonians. Quantum computers typically support only two-qubit gates. However, it is possible to approximately map any many-body interaction Hamiltonian to two-body Hamiltonian using the concept of perturbative gadgets~\cite{Kempe:2006, Jordan:2008, Bravyi:2008, Babbush:2014}.


Quantum mechanical embedding methods hold the promise to transform not just the way calculations are performed,
but to significantly reduce computational costs and improve scaling for macro-molecular systems containing hundreds if not
thousands of atoms.

In complex systems, it is often the case that the region of interest forms only one part of a much larger system. The idea of joining two different quantum simulations—a high level calculation on the active region of interest, and a low level calculation on its environment—formally defines a quantum embedding

 another approach is to subdivide the
system of interest, compute the smaller subsystems, then
combine the pieces. This has been shown to be highly effective,
and such techniques are commonly called quantum embeddingthe act of embedding a smaller system of interest in a
larger one (surrounding environment)

Quantum embedding (QE) methods aim to reduce the
computational cost of a large calculation by dividing up an
atomic or molecular ensemble into smaller less-costly
subsystems; the overall cost of calculating and combining
these subsystems should be less than the cost of a single
calculation of the whole system

Thus, in
some QE theories it is crucial to avoid breaking bonds
(hydrogen bonds, covalent, ionic, π−π, etc.), which are
important to the physical properties of the system one is
trying to understand

An important aspect of embedding models is the ability to
“mix and match” different levels of theory.

The idea is to use a
good level for the fragment of interest and use a lower level for
the surrounding environment.

unfortunately this limited number of qubits still prevents straightforward quantum simulations of realistic molecules and materials, whose description requires hundreds of atoms and thousands to millions of degrees of freedom to represent the electronic wavefunctions. An important requirement to tackle complex chemistry and material science problems using NISQ computers is the reduction of the number of electrons treated explicitly at the highest level of accuracy \cite{rubin2016hybrid, bauer2016hybrid}

While it has been shown that such a quantum computer can in principle solve
certain small electronic structure problems and idealized model Hamiltonians, the highly relevant problem
of directly solving a complex correlated material appears to require a prohibitive amount of resources.
using a hybrid quantum-classical algorithm that incorporates the power of a small quantum
computer into a framework of classical embedding algorithms, the electronic structure of complex
correlated materials can be efficiently tackled using a quantum computer.
the quantum
computer solves a small effective quantum impurity problem that is self-consistently determined via a
feedback loop between the quantum and classical computation. Use of a quantum computer enables much
larger and more accurate simulations than with any known classical algorithm, and will allow many open
questions in quantum materials to be resolved once a small quantum computer with around 100 logical
qubits becomes available


one may simplify complex molecular and material science problems by defining active regions (or building blocks) with strongly-correlated electronic states, embedded in an environment that may be described within mean-field theory






% In particular, given the huge demand for smaller, faster, and lower-power devices with potential for favorable capabilities such as flexibility and transparency, the need to discover and better understand quantum materials is essential. 

%The last decade has seen enormous advances in quantum hardware, with parallel advancement of both algorithm and software development, which are beginning to enable simulation of quantum materials on DQCs. 

